HackAtari: Atari Learning Environments for Robust and Continual Reinforcement Learning

Artificial agents' adaptability to novelty and alignment with intended behavior is crucial for their effective deployment. Reinforcement learning (RL) leverages novelty as a means of exploration, yet agents often struggle to handle novel situations, hindering generalization. To address these issues, we propose HackAtari, a framework introducing controlled novelty to the most common RL benchmark, the Atari Learning Environment. HackAtari allows us to create novel game scenarios (including simplification for curriculum learning), to swap the game elements' colors, as well as to introduce different reward signals for the agent. We demonstrate that current agents trained on the original environments include robustness failures, and evaluate HackAtari's efficacy in enhancing RL agents' robustness and aligning behavior through experiments using C51 and PPO. Overall, HackAtari can be used to improve the robustness of current and future RL algorithms, allowing Neuro-Symbolic RL, curriculum RL, causal RL, as well as LLM-driven RL. Our work underscores the significance of developing interpretable in RL agents.

==> environment_description/Alien.tex <==
You are stuck in a maze-like space ship with three aliens. You goal is to destroy their eggs that are scattered all over the ship while simultaneously avoiding the aliens (they are trying to kill you). You have a flamethrower that can help you turn them away in tricky situations. Moreover, you can occasionally collect a power-up (pulsar) that gives you the temporary ability to kill aliens.

==> environment_description/Amidar.tex <==
This game is similar to Pac-Man: You are trying to visit all places on a 2-dimensional grid while simultaneously avoiding your enemies. You can turn the tables at one point in the game: Your enemies turn into chickens and you can catch them.

==> environment_description/Assault.tex <==
You control a vehicle that can move sideways. A big mother ship circles overhead and continually deploys smaller drones. You must destroy these enemies and dodge their attacks.

==> environment_description/Asterix.tex <==
You are Asterix and can move horizontally (continuously) and vertically (discretely). Objects move horizontally across the screen: lyres and other (more useful) objects. Your goal is to guide Asterix in such a way as to avoid lyres and collect as many other objects as possible. You score points by collecting objects and lose a life whenever you collect a lyre. You have three lives available at the beginning. If you score sufficiently many points, you will be awarded additional points.

==> environment_description/Asteroids.tex <==
This is a well-known arcade game: You control a spaceship in an asteroid field and must break up asteroids by shooting them. Once all asteroids are destroyed, you enter a new level and new asteroids will appear. You will occasionally be attacked by a flying saucer.

==> environment_description/Atlantis.tex <==
Your job is to defend the submerged city of Atlantis. Your enemies slowly descend towards the city and you must destroy them before they reach striking distance. To this end, you control three defense posts. You lose if your enemies manage to destroy all seven of Atlantis’ installations. You may rebuild installations after you have fought of a wave of enemies and scored a sufficient number of points.

==> environment_description/Berzerk.tex <==
You are stuck in a maze with evil robots. You must destroy them and avoid touching the walls of the maze, as this will kill you. You may be awarded extra lives after scoring a sufficient number of points, depending on the game mode. You may also be chased by an undefeatable enemy, Evil Otto, that you must avoid. Evil Otto does not appear in the default mode.

==> environment_description/Bowling.tex <==
Your goal is to score as many points as possible in the game of Bowling. A game consists of 10 frames and you have two tries per frame. Knocking down all pins on the first try is called a “strike”. Knocking down all pins on the second roll is called a “spar”. Otherwise, the frame is called “open”.

==> environment_description/Centipede.tex <==
You are an elf and must use your magic wands to fend off spiders, fleas and centipedes. Your goal is to protect mushrooms in an enchanted forest. If you are bitten by a spider, flea or centipede, you will be temporally paralyzed and you will lose a magic wand. The game ends once you have lost all wands. You may receive additional wands after scoring a sufficient number of points.

==> environment_description/CrazyClimber.tex <==
You are a climber trying to reach the top of four buildings, while avoiding obstacles like closing windows and falling objects. When you receive damage (windows closing or objects) you will fall and lose one life; you have a total of 5 lives before the end games. At the top of each building, there’s a helicopter which you need to catch to get to the next building. The goal is to climb as fast as possible while receiving the least amount of damage.

==> environment_description/DemonAttack.tex <==
You are facing waves of demons in the ice planet of Krybor. Points are accumulated by destroying demons. You begin with 3 reserve bunkers, and can increase its number (up to 6) by avoiding enemy attacks. Each attack wave you survive without any hits, grants you a new bunker. Every time an enemy hits you, a bunker is destroyed. When the last bunker falls, the next enemy hit will destroy you and the game ends.

==> environment_description/Gopher.tex <==
The player controls a shovel-wielding farmer who protects a crop of three carrots from a gopher.

==> environment_description/Hero.tex <==
You need to rescue miners that are stuck in a mine shaft. You have access to various tools: A propeller backpack that allows you to fly wherever you want, sticks of dynamite that can be used to blast through walls, a laser beam to kill vermin, and a raft to float across stretches of lava.You have a limited amount of power. Once you run out, you lose a live.

==> environment_description/IceHockey.tex <==
Your goal is to score as many points as possible in a standard game of Ice Hockey over a 3-minute time period. The ball is usually called “the puck”.There are 32 shot angles ranging from the extreme left to the extreme right. The angles can only aim towards the opponent’s goal.Just as in real hockey, you can pass the puck by shooting it off the sides of the rink. This can be really key when you’re in position to score a goal.

==> environment_description/Jamesbond.tex <==
Your mission is to control Mr. Bond’s specially designed multipurpose craft to complete a variety of missions.The craft moves forward with a right motion and slightly back with a left motion.An up or down motion causes the craft to jump or dive.You can also fire by either lobbing a bomb to the bottom of the screen or firing a fixed angle shot to the top of the screen.

==> environment_description/Krull.tex <==
Your mission is to find and enter the Beast’s Black Fortress, rescue Princess Lyssa, and destroy the Beast.The task is not an easy one, for the location of the Black Fortress changes with each sunrise on Krull.

==> environment_description/Pacman.tex <==
A classic arcade game. Move Pac Man around a maze collecting food and avoiding ghosts- unless you eat a Power Pellet, then you can eat the ghosts too!

==> environment_description/Pitfall.tex <==
You control Pitfall Harry and are tasked with collecting all the treasures in a jungle within 20 minutes. You have three lives. The game is over if you collect all the treasures or if you die or if the time runs out.

==> environment_description/PrivateEye.tex <==
You control the French Private Eye Pierre Touche. Navigate the city streets, parks, secret passages, dead-ends and one-ways in search of the ringleader, Henri Le Fiend and his gang. You also need to find evidence and stolen goods that are scattered about. There are five cases, complete each case before its statute of limitations expires.

==> environment_description/Qbert.tex <==
You are Q*bert. Your goal is to change the color of all the cubes on the pyramid to the pyramid’s ‘destination’ color. To do this, you must hop on each cube on the pyramid one at a time while avoiding nasty creatures that lurk there.

==> environment_description/Riverraid.tex <==
You control a jet that flies over a river: you can move it sideways and fire missiles to destroy enemy objects. Each time an enemy object is destroyed you score points (i.e. rewards). You lose a jet when you run out of fuel: fly over a fuel depot when you begin to run low.You lose a jet even when it collides with the river bank or one of the enemy objects (except fuel depots). The game begins with a squadron of three jets in reserve and you’re given an additional jet (up to 9) for each 10,000 points you score.

==> environment_description/RoadRunner.tex <==
You control the Road Runner(TM) in a race; you can control the direction to run in and times to jumps.The goal is to outrun Wile E. Coyote(TM) while avoiding the hazards of the desert.The game begins with three lives. You lose a life when the coyote catches you, picks you up in a rocket, or shoots you with a cannon. You also lose a life when a truck hits you, you hit a land mine, you fall off a cliff,or you get hit by a falling rock.You score points (i.e. rewards) by eating seeds along the road, eating steel shot, and destroying the coyote.

==> environment_description/TimePilot.tex <==
You control an aircraft. Use it to destroy your enemies. As you progress in the game, you encounter enemies with technology that is increasingly from the future.

==> environment_description/UpNDown.tex <==
Your goal is to steer your baja bugger to collect prizes and eliminate opponents.

==> environment_description/Venture.tex <==
Your goal is to capture the treasure in every chamber of the dungeon while eliminating the monsters.

==> environment_description/VideoPinball.tex <==
Your goal is to keep the ball in play as long as possible and to score as many points as possible.

==> environment_description/YarsRevenge.tex <==
The objective is to break a path through the shield and destroy the Qotile with a blast from the Zorlon Cannon.

==> neurips_checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}, Our paper introduces a new framework to test and benchmark Atari agents. The claims are clearly stated in the introduction and are further elaborated in our methodology section (\cf Sections~\ref{sec:Hackatari} and~\ref{sec:paradigm}) and experimental evaluation (\cf Section~\ref{sec:experiments}). Further are the claims discussed in Section~\ref{sec:limitations}.  
  \item Did you describe the limitations of your work?
    \answerYes{}, Limitations are stated and discussed in the Section~\ref{sec:limitations}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}, We provide these together with ethical consideration and a statement about broader impact in the paper (\cf Section~\ref{sec:ethics}).
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}, We provide two anonynmous repositories (HackAtari, CleanRL) including the code as well as a ReadMe giving instructions to reproduce our experiments. We did not use any data set or pre-trained agents. Hyperparameters and seeds for the algorithm/frameworks/evaluation are given in the Appendix. Further we provide some example scripts how we trained our agents and evaluated them. A selected subset of models trained can also be found in the supplementary materials to test performance and reproduce our evaluation. 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}, all necessary information about hyperparameters and the experimental setup can in Section~\ref{sec:experiments} and Section~\ref{app:hyperparameter}. We use the parameters as described by CleanRL~\citep{huang2022cleanrl}. We do not provide any hyperparameter optimization and used the default set, as can be seen in the anonymous fork.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}, Each experiment is done with 3 seeds. The error bars display the standard variation over a running window, while the figures display the mean between all seeds. To mitigate noise and fluctuations, we use exponential moving average (EMA) smoothing in all curves. The process is explained in the Appendix. 
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}, We provide computational information, \ie. hardware and software specifications (\cf Section~\ref{app:hyperparameter}), in the Appendix. We do not provide the individual computational costs, like time of execution but a sum of them. 
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{},  We cite prior work, respectively. The codebase we are using (CleanRL, ALE, Gymnasium) are openly accessible and cited properly. 
  \item Did you mention the license of the assets?
    \answerYes{}, all of our code will be published and be openly accessible. 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}, we provide links to all of our code in form of anonymous git repositories. A subset of models is also given in the supplements to make reproduciblity and testing the environment easier.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}, we do not use any data set or pre-trained agents. All code we are using is openly accessible or under GPL license.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{}, we are discussing that in the paper (\cf Section~\ref{sec:ethics}.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{}, We evaluated human performance on a subset on new game variations. The complete list of instructions as well as provided information is given in the supplement materials and explained in Section~\ref{app:human_eval}. There was no compensation. 
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{} The participants of our study were informed about potential risks, goal of the study, usage of the collected data. All participants had to give their consents before taking part. Withdrawal was possible at all time. We follow the guidelines of the institutional ethics commission. The consent form can be found in the supplements. 
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{}, participants were not compensated for the user study as mentioned in Section~\ref{app:human_eval}.
\end{enumerate}

\end{enumerate}

\clearpage

==> reports/BankHeist.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | p{10cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        unlimited\_gas & Unlimited gas all the enemies.  \\
        no\_police & Removes police from the game.\\
        only\_police & No banks only police. \\
        random\_city & Randomizes which city is entered next. \\
        revisit\_city & Allows player to go back one city. \\ \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}

==> reports/Battlezone.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | p{10cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        no\_radar &  Removes the radar content.  \\
        
    \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}


==> reports/Seaquest.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{4cm} | p{9cm}} \toprule
        \textbf{Modification} & \textbf{Effect} \\ \midrule
        unlimited\_oxygen & Changes the behavior of the oxygen bar to remain filled\\
        gravity & Enables gravity for the player. \\
        disable\_enemies &  Disables all the enemies.\\
        random\_color\_enemies & The enemies have new random colors each time they go across the screen. \\
        \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}

==> reports/SpaceInvaders.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{p{3cm} | m{2cm} | p{8cm}} \toprule
        \textbf{Modification} & \textbf{Parameter} & \textbf{Effect} \\ \midrule
        disable\_shield\_left && Disables the left shield.\\
        disable\_shield\_middle && Disables the middle shield.\\
        disable\_shield\_right && Disables the right shield.\\
        disable\_shields && Disables all shields.\\
        curved && Makes the shots travel on a curved path.\\
        relocate$XX$ &$X \in (35,53)$& Allows for the relocation of the shields via an offset. \\
        
        \bottomrule
    \end{tabular}
    % \label{tab:my_label}
\end{table}
